A Fourier State Space Model for Bayesian ODE Filters

Gaussian ODE filtering is a probabilistic numerical method to solve ordinary differential equations (ODEs). It computes a Bayesian posterior over the solution from evaluations of the vector field defining the ODE. Its most popular version, which employs an integrated Brownian motion prior, uses Taylor expansions of the mean to extrapolate forward and has the same convergence rates as classical numerical methods. As the solution of many important ODEs are periodic functions (oscillators), we raise the question whether Fourier expansions can also be brought to bear within the framework of Gaussian ODE filtering. To this end, we construct a Fourier state space model for ODEs and a `hybrid' model that combines a Taylor (Brownian motion) and Fourier state space model. We show by experiments how the hybrid model might become useful in cheaply predicting until the end of the time domain.

==> fig/TEX_lv_opt.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}[trim axis left,trim axis right,baseline]

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

% \begin{groupplot}[group style={group size=2 by 1}]
\begin{groupplot}[group style={group size=1 by 1}]

\nextgroupplot[
width=\figwidth,
height=\figheight,
scale only axis,
% width=0.3\textwidth,
legend style={at={(0,0)}, xshift=0.15cm, yshift=0.05cm, anchor=south west },
ymode=log,
ylabel={Neg. log-likelihood},
% title = {\bf Optimization}
]
\addplot+
table {%
0 1393098.95998807
1 1393098.95998807
2 1365859.80514612
3 1365859.80514612
4 1365859.80514612
5 1365859.80514612
6 1365859.80514612
7 1352070.20091395
8 1352070.20091395
9 1352070.20091395
10 1352070.20091395
11 1311388.26151442
12 1311388.26151442
13 1236501.54594476
14 1236501.54594476
15 1236501.54594476
16 1185368.71247196
17 1185368.71247196
18 1185368.71247196
19 1185368.71247196
20 1185368.71247196
21 1082060.50200496
22 1082060.50200496
23 1082060.50200496
24 1082060.50200496
25 1082060.50200496
26 1082060.50200496
27 1049762.52403809
28 952490.329864678
29 952490.329864678
30 952490.329864678
31 952490.329864678
32 832550.814325873
33 779712.756222619
34 776359.357103089
35 722430.922418072
36 722430.922418072
37 645134.153492063
38 578699.92921578
39 492371.988754658
40 381922.382748681
41 381922.382748681
42 381922.382748681
43 355413.945745475
44 355413.945745475
45 355413.945745475
46 355413.945745475
47 355413.945745475
48 355413.945745475
49 355413.945745475
};
\addlegendentry{RS}
\addplot+
table {%
0 1393098.95998807
1 1090605.53183751
2 821637.586886575
3 593264.615703072
4 421713.758066416
5 328239.616831898
6 331424.596552061
7 416450.097049457
8 457093.064699312
9 236721.769535925
10 134257.987476327
11 156029.929407882
12 65755.3677595245
13 40390.9268152136
14 57273.5929519011
15 53193.6242778977
16 18673.2210106684
17 9209.18171685116
18 8380.07006718789
19 6717.00296067827
20 10738.0992503794
21 12535.6434538686
22 8016.68885952329
23 3954.7741086071
24 3132.78676607872
25 3802.55662494184
26 5247.47520442604
27 6148.5641834069
28 5596.1063787733
29 4496.34190684225
30 3937.7794651198
31 4052.46527765143
32 4510.33579995626
33 4869.96062804102
34 4854.21108070214
35 4582.53358286371
36 4353.89513763679
37 4320.07867144746
38 4433.98696297984
39 4558.62014549748
40 4590.00336552147
41 4529.02251856823
42 4450.0561033425
43 4416.24227936395
44 4434.56667458476
45 4470.4106088126
46 4487.04158784429
47 4474.30875874768
48 4448.20305647906
49 4429.80745202906
};
\addlegendentry{GD}
\addplot+
table {%
0 1393098.95998807
1 1085013.96608212
2 833645.135401544
3 615009.459950509
4 433326.70872668
5 295122.861999796
6 212949.009719144
7 152289.640306393
8 82940.6641475305
9 63679.5966834178
10 51458.9908232228
11 42870.536941719
12 35373.7587424317
13 28139.6168890103
14 21217.2703160641
15 15012.6064117364
16 9924.01185339072
17 6125.77981277611
18 3534.92430245974
19 1908.05625525718
20 961.907919390796
21 451.106925527424
22 195.891061977816
23 79.0284908345459
24 30.9139241152886
25 13.6745520050523
26 8.53893470132973
27 7.21208377866428
28 6.59538867416741
29 5.8582122167199
30 4.97926672375324
31 4.11516270051029
32 3.38422155708475
33 2.82943049459369
34 2.44060504230154
35 2.18393996260732
36 2.02227273891673
37 1.92467370829928
38 1.86882095238484
39 1.83986082721177
40 1.82824403745247
41 1.82777341098256
42 1.83425351029056
43 1.84470434915806
44 1.85695848119736
45 1.86946486014208
46 1.88117890037196
47 1.89147570394087
48 1.90006369851997
49 1.90689735173486
};
\addlegendentry{NWT}
\end{groupplot}

\end{tikzpicture}


% \nextgroupplot[
% axis line style={white!80!black},
% log basis y={10},
% tick align=outside,
% tick pos=left,
% title={Distance to true parameter},
% x grid style={white!80!black},
% xmajorgrids,
% xmin=-2.45, xmax=51.45,
% xtick style={color=white!15!black},
% y grid style={white!80!black},
% ymajorgrids,
% ymin=0.00106073763964196, ymax=4.11487678045554,
% ymode=log,
% ytick style={color=white!15!black},
% ytick={0.0001,0.001,0.01,0.1,1,10,100},
% yticklabels={\(\displaystyle {10^{-4}}\),\(\displaystyle {10^{-3}}\),\(\displaystyle {10^{-2}}\),\(\displaystyle {10^{-1}}\),\(\displaystyle {10^{0}}\),\(\displaystyle {10^{1}}\),\(\displaystyle {10^{2}}\)}
% ]
% \addplot [ultra thick, color0]
% table {%
% 0 1.14017542509914
% 1 1.14017542509914
% 2 1.07653319681145
% 3 1.07653319681145
% 4 1.07653319681145
% 5 1.07653319681145
% 6 1.07653319681145
% 7 1.10498440528307
% 8 1.10498440528307
% 9 1.10498440528307
% 10 1.10498440528307
% 11 1.03143801002773
% 12 1.03143801002773
% 13 0.952426837335556
% 14 0.952426837335556
% 15 0.952426837335556
% 16 0.879504877170528
% 17 0.879504877170528
% 18 0.879504877170528
% 19 0.879504877170528
% 20 0.879504877170528
% 21 0.792622914543451
% 22 0.792622914543451
% 23 0.792622914543451
% 24 0.792622914543451
% 25 0.792622914543451
% 26 0.792622914543451
% 27 0.78892087553874
% 28 0.731269806388593
% 29 0.731269806388593
% 30 0.731269806388593
% 31 0.731269806388593
% 32 0.658215058981417
% 33 0.625517784427277
% 34 0.627324586931649
% 35 0.625894936609278
% 36 0.625894936609278
% 37 0.552986753194924
% 38 0.544289147143617
% 39 0.473742745334361
% 40 0.401152922904796
% 41 0.401152922904796
% 42 0.401152922904796
% 43 0.389379622300786
% 44 0.389379622300786
% 45 0.389379622300786
% 46 0.389379622300786
% 47 0.389379622300786
% 48 0.389379622300786
% 49 0.389379622300786
% };
% \addplot [ultra thick, color1]
% table {%
% 0 1.14017542509914
% 1 0.972534525116298
% 2 0.840853224962363
% 3 0.754481586621778
% 4 0.711678395246213
% 5 0.69521937631633
% 6 0.675966298883208
% 7 0.621123697662269
% 8 0.507963354236103
% 9 0.377557538563487
% 10 0.345498990605347
% 11 0.245874691560426
% 12 0.229572706541314
% 13 0.28160957158844
% 14 0.312105684301101
% 15 0.30523141239397
% 16 0.281827281738267
% 17 0.252803350075906
% 18 0.232779224058443
% 19 0.24254180590126
% 20 0.260362266222557
% 21 0.267714331808638
% 22 0.263823129739471
% 23 0.25477017811667
% 24 0.247866902593619
% 25 0.24815238615114
% 26 0.252999159380693
% 27 0.256724703872284
% 28 0.256856632335079
% 29 0.254458580527256
% 30 0.252016222928375
% 31 0.251362300036042
% 32 0.252382464372475
% 33 0.253648063440012
% 34 0.254038072626329
% 35 0.253489530005667
% 36 0.252662694487828
% 37 0.252219396510996
% 38 0.252317790712189
% 39 0.252642532121938
% 40 0.25280734805163
% 41 0.252678469766196
% 42 0.252390764008121
% 43 0.252156584055668
% 44 0.252078509915379
% 45 0.252105360685116
% 46 0.252121846374372
% 47 0.252058774802065
% 48 0.251930912178281
% 49 0.251797985719012
% };
% \addplot [ultra thick, color2]
% table {%
% 0 1.14017542509914
% 1 1.18336386613828
% 2 1.49392570244984
% 3 1.71473150104136
% 4 2.22857638364891
% 5 2.82638869205517
% 6 2.25296766652401
% 7 0.655897287756813
% 8 0.362919883910724
% 9 0.442537022314815
% 10 0.520580550652745
% 11 0.550458232140984
% 12 0.538114710698247
% 13 0.494223022226252
% 14 0.430681226183816
% 15 0.358516977023748
% 16 0.286503921725002
% 17 0.220546624027821
% 18 0.163802612337358
% 19 0.117291932700225
% 20 0.0806516346360732
% 21 0.0527820614365598
% 22 0.032291999422822
% 23 0.0177618951550297
% 24 0.00788246296720637
% 25 0.00154430446731801
% 26 0.00236675313237788
% 27 0.00439170615629489
% 28 0.00523958270438084
% 29 0.00534903573919486
% 30 0.00504305881632753
% 31 0.00454522587858311
% 32 0.00400088202633356
% 33 0.00349628165834663
% 34 0.00307491421788762
% 35 0.00275111611235615
% 36 0.00252125279037389
% 37 0.00237247289113385
% 38 0.00228876914472399
% 39 0.00225439393467135
% 40 0.0022553229158506
% 41 0.00227970339723185
% 42 0.00231792839554834
% 43 0.00236257694572966
% 44 0.00240825668641381
% 45 0.00245135364703694
% 46 0.00248971788558575
% 47 0.00252232779887498
% 48 0.00254897158395659
% 49 0.00256997107921563
% };

